Combining Human Predictions with Model Probabilities via Confusion Matrices and Calibration

An increasingly common use case for machine learning models is augmenting the abilities of human decision makers. For classification tasks where neither the human or model are perfectly accurate, a key step in obtaining high performance is combining their individual predictions in a manner that leverages their relative strengths. In this work, we develop a set of algorithms that combine the probabilistic output of a model with the class-level output of a human. We show theoretically that the accuracy of our combination model is driven not only by the individual human and model accuracies, but also by the model's confidence. Empirical results on image classification with CIFAR-10 and a subset of ImageNet demonstrate that such human-model combinations consistently have higher accuracies than the model or human alone, and that the parameters of the combination method can be estimated effectively with as few as ten labeled datapoints.

==> misc/scrap.tex <==
%%%%%%%%  Old version of estimation error lemma
For a given $x$, the posterior $p(Y = i | h(x) = j, m(x))$ is approximated in our combination model by $C_i(X) = \widehat{\psi}_{ji} \widehat{m}_i(x)$. Let $\eta_{ij}(X) = ||P(Y = i | h(X) = j, m(X)) - C_i(X)||$ be the estimation error between the output of our combiner $C(X)$ and the true posterior. 

The following lemma shows us that we can upper bound our estimation error by the estimation error for the confusion matrix and (a variant of) the calibration error. (With sufficient data, it should be possible to have $\widehat{\psi}_{ij} \to \psi_{ij}$, i.e. the confusion matrix error term goes to zero. This isn't necessarily true for calibration though, due to e.g. the limited expressiveness of our calibration map. This lemma shows us how that's reflected in the combination.)

\begin{theorem}
Suppose that $Y = i$ and $h(X) = j$. Then, the expected posterior error $\Exp[X]{\eta_{ij}(X)}$ is bounded by the sum of the error in the confusion matrix at entry $ji$ and the calibration error conditioned on $Y = i$:
\begin{align}
    \Exp[X | Y = i, h(X) = j]{\eta_{ij}(X)} \leq ||\psi_{ji} - \widehat{\psi}_{ji} || + \Exp[X | Y = i, h(X) = j]{||P(Y = i | m(X)) - \widehat{m}_i(X) ||}
\end{align}
\end{theorem}
%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%% Full version of Noisy ImageNet results
\begin{table}[!h]
\begin{tabular}{lllllll}
\toprule
\multicolumn{2}{c}{} &
\multicolumn{5}{c}{Combination} \\
\cmidrule(lr){3-7}
        Human & Model &   Confusion &    Uncalibrated &       TS &      ETS & IMax \\
\midrule
9.85& $23.01 \pm 1.22$ &  $9.19 \pm 0.59$ &  $9.26 \pm 0.70$ &  $8.48 \pm 0.68$ &  $\bm{8.43 \pm 0.72}$ &  $8.46 \pm 0.64$ \\
--- & $21.00 \pm 0.90$ &  $\bm{8.15 \pm 0.41}$ &  $8.37 \pm 0.60$ &  $8.50 \pm 0.64$ &  $8.52 \pm 0.65$ &  $8.57 \pm 0.70$ \\
--- & $10.72 \pm 0.95$ &  $\bm{6.39 \pm 0.62}$ &  $6.45 \pm 0.61$ &  $6.48 \pm 0.65$ &  $6.57 \pm 0.63$ &  $6.74 \pm 0.60$ \\
\midrule
14.07 & $38.25 \pm 1.00$ & $13.17 \pm 0.62$ & $15.03 \pm 0.67$ & $13.59 \pm 0.68$ & $13.52 \pm 0.76$ & $\bm{13.14 \pm 0.67}$ \\
--- & $25.83 \pm 1.11$ & $\bm{11.40 \pm 0.59}$ & $12.17 \pm 0.77$ & $12.50 \pm 0.74$ & $12.47 \pm 0.68$ & $12.81 \pm 0.73$ \\
--- & $13.43 \pm 0.55$ &  $9.42 \pm 0.52$ &  $\bm{8.82 \pm 0.51}$ &  $8.95 \pm 0.50$ &  $8.99 \pm 0.51$ &  $9.85 \pm 0.62$ \\
\midrule
23.34 & $62.33 \pm 1.61$ & $\bm{23.18 \pm 0.86}$ & $29.33 \pm 1.11$ & $23.74 \pm 0.94$ & $23.85 \pm 0.87$ & $23.37 \pm 0.77$ \\
--- & $32.13 \pm 1.28$ & $19.46 \pm 0.98$ & $\bm{19.11 \pm 1.17}$ & $19.30 \pm 1.03$ & $19.28 \pm 1.08$ & $19.75 \pm 0.90$ \\
--- & $17.55 \pm 0.88$ & $14.48 \pm 0.84$ & $13.92 \pm 1.01$ & $\bm{14.05 \pm 1.02}$ & $14.10 \pm 1.05$ & $15.01 \pm 1.01$ \\
\midrule
39.77 & $85.18 \pm 0.59$ & $\bm{39.39 \pm 0.98}$ & $60.28 \pm 1.03$ & $39.65 \pm 0.97$ & $39.51 \pm 0.96$ & $39.72 \pm 0.97$ \\
--- & $39.31 \pm 1.06$ & $31.37 \pm 1.06$ & $\bm{30.61 \pm 0.86}$ & $31.19 \pm 0.92$ & $31.31 \pm 0.95$ & $32.37 \pm 0.84$ \\
--- & $25.74 \pm 1.19$ & $23.87 \pm 1.36$ & $\bm{21.60 \pm 0.98}$ & $21.99 \pm 0.94$ & $22.20 \pm 0.89$ & $24.27 \pm 1.05$ \\
\bottomrule \\
\end{tabular}
\caption{Noisy ImageNet error rates (DenseNet-164)}
\end{table}


\begin{table}[!h]
\centering
\begin{tabular}{llll}
\toprule
          Model &              TS &             ETS &        IMax \\
\midrule
$1.58 \pm 0.09$ & $1.62 \pm 0.08$ & $1.62 \pm 0.09$ & $2.42 \pm 0.06$ \\
$1.92 \pm 0.13$ & $2.00 \pm 0.12$ & $2.02 \pm 0.11$ & $2.71 \pm 0.08$ \\
$1.00 \pm 0.08$ & $1.03 \pm 0.08$ & $1.06 \pm 0.08$ & $1.84 \pm 0.11$ \\
\midrule
$2.59 \pm 0.07$ & $2.49 \pm 0.07$ & $2.50 \pm 0.07$ & $3.17 \pm 0.07$ \\
$2.21 \pm 0.11$ & $2.26 \pm 0.11$ & $2.27 \pm 0.11$ & $2.99 \pm 0.06$ \\
$1.12 \pm 0.05$ & $1.17 \pm 0.05$ & $1.18 \pm 0.06$ & $2.00 \pm 0.06$ \\
\midrule
$4.34 \pm 0.13$ & $3.79 \pm 0.10$ & $3.80 \pm 0.09$ & $3.89 \pm 0.06$ \\
$2.54 \pm 0.12$ & $2.57 \pm 0.12$ & $2.60 \pm 0.11$ & $3.21 \pm 0.07$ \\
$1.36 \pm 0.09$ & $1.40 \pm 0.09$ & $1.42 \pm 0.09$ & $2.22 \pm 0.11$ \\
\midrule
$6.48 \pm 0.14$ & $4.09 \pm 0.14$ & $4.09 \pm 0.18$ & $3.39 \pm 0.15$ \\
$2.79 \pm 0.10$ & $2.82 \pm 0.09$ & $2.83 \pm 0.09$ & $3.38 \pm 0.11$ \\
$1.80 \pm 0.08$ & $1.84 \pm 0.08$ & $1.87 \pm 0.08$ & $2.70 \pm 0.08$ \\
\bottomrule
\end{tabular}

\caption{Calibration error of the model (pre- and post- calibration, DenseNet-164)}
\end{table}

\begin{table}[!h]
    \centering
    \begin{tabular}{lllll}
\toprule
       Confusion &         Uncalibrated &            TS &           ETS &      IMax \\
    \midrule
    $0.99 \pm 0.08$ & $0.66 \pm 0.05$ & $0.58 \pm 0.06$ & $0.58 \pm 0.06$ & $0.54 \pm 0.06$ \\
    $0.90 \pm 0.06$ & $0.64 \pm 0.06$ & $0.58 \pm 0.07$ & $0.58 \pm 0.07$ & $0.57 \pm 0.07$ \\
    $0.66 \pm 0.07$ & $0.47 \pm 0.05$ & $0.46 \pm 0.05$ & $0.46 \pm 0.05$ & $0.45 \pm 0.04$ \\
    $1.45 \pm 0.07$ & $1.13 \pm 0.07$ & $0.96 \pm 0.07$ & $0.95 \pm 0.08$ & $0.85 \pm 0.07$ \\
    $1.25 \pm 0.04$ & $0.91 \pm 0.09$ & $0.84 \pm 0.10$ & $0.84 \pm 0.09$ & $0.82 \pm 0.10$ \\
    $0.93 \pm 0.03$ & $0.59 \pm 0.07$ & $0.58 \pm 0.07$ & $0.57 \pm 0.07$ & $0.59 \pm 0.07$ \\
    $2.23 \pm 0.08$ & $2.09 \pm 0.12$ & $1.42 \pm 0.09$ & $1.46 \pm 0.10$ & $1.26 \pm 0.11$ \\
    $1.88 \pm 0.12$ & $1.38 \pm 0.13$ & $1.27 \pm 0.12$ & $1.26 \pm 0.12$ & $1.19 \pm 0.11$ \\
    $1.36 \pm 0.09$ & $0.89 \pm 0.08$ & $0.87 \pm 0.08$ & $0.86 \pm 0.08$ & $0.86 \pm 0.09$ \\
    $2.98 \pm 0.09$ & $4.64 \pm 0.17$ & $1.97 \pm 0.12$ & $2.09 \pm 0.12$ & $1.66 \pm 0.14$ \\
    $2.67 \pm 0.07$ & $1.99 \pm 0.07$ & $1.79 \pm 0.07$ & $1.77 \pm 0.07$ & $1.67 \pm 0.09$ \\
    $2.17 \pm 0.09$ & $1.31 \pm 0.09$ & $1.28 \pm 0.09$ & $1.26 \pm 0.09$ & $1.23 \pm 0.08$ \\
    \bottomrule \\
    \end{tabular}
    \caption{Calibration error ($10^{-2}$) of the combined predictions on Noisy ImageNet (DenseNet-164). Lower is better.}
\end{table}

\begin{table}[!h]
\begin{tabular}{lllllll}
\toprule
\multicolumn{2}{c}{} &
\multicolumn{5}{c}{Combination} \\
\cmidrule(lr){3-7}
       Human & Model &   Confusion &    Uncalibrated &       TS &      ETS & IMax \\
\midrule
9.85 & $16.91 \pm 1.15$ &  $\bm{7.45 \pm 0.41}$ &  $8.23 \pm 0.58$ &  $8.15 \pm 0.50$ &  $8.16 \pm 0.52$ &   $8.06 \pm 0.55$ \\
--- & $11.70 \pm 0.80$ &  $6.92 \pm 0.48$ &  $6.55 \pm 0.49$ &  $6.66 \pm 0.55$ &  $6.62 \pm 0.54$ &   $\bm{6.62 \pm 0.57}$ \\
--- & $11.03 \pm 0.89$ &  $6.49 \pm 0.56$ &  $7.34 \pm 0.58$ &  $6.38 \pm 0.60$ &  $6.50 \pm 0.58$ &   $\bm{5.97 \pm 0.49}$ \\
\midrule
14.07 & $22.00 \pm 0.94$ & $\bm{11.04 \pm 0.58}$ & $12.10 \pm 0.65$ & $12.33 \pm 0.72$ & $12.24 \pm 0.67$ &  $12.13 \pm 0.63$ \\
--- & $15.46 \pm 0.96$ & $10.43 \pm 0.66$ &  $\bm{9.69 \pm 0.67}$ & $10.06 \pm 0.67$ & $10.07 \pm 0.63$ &  $10.07 \pm 0.64$ \\
--- & $12.82 \pm 0.92$ &  $9.15 \pm 0.62$ &  $9.08 \pm 0.55$ &  $9.07 \pm 0.59$ &  $9.20 \pm 0.59$ &   $\bm{8.40 \pm 0.63}$ \\
\midrule
23.34 & $29.65 \pm 1.27$ & $19.29 \pm 0.95$ & $19.57 \pm 0.98$ & $19.19 \pm 0.93$ & $19.50 \pm 0.95$ &  $\bm{19.15 \pm 0.99}$ \\
--- & $22.14 \pm 0.99$ & $16.55 \pm 0.80$ & $\bm{15.22 \pm 0.94}$ & $15.60 \pm 0.98$ & $16.12 \pm 1.01$ & $37.82 \pm 19.47$ \\
--- & $15.85 \pm 0.73$ & $14.23 \pm 0.83$ & $12.64 \pm 0.76$ & $13.10 \pm 0.85$ & $13.18 \pm 0.88$ &  $\bm{12.27 \pm 0.78}$ \\
\midrule
39.77 & $44.17 \pm 1.00$ & $\bm{33.26 \pm 1.17}$ & $34.76 \pm 1.14$ & $34.47 \pm 1.15$ & $34.63 \pm 1.06$ &  $34.94 \pm 3.46$ \\
--- & $34.24 \pm 1.03$ & $28.58 \pm 1.11$ & $\bm{27.31 \pm 0.94}$ & $28.21 \pm 1.01$ & $28.73 \pm 0.97$ &  $28.07 \pm 1.01$ \\
--- & $21.68 \pm 0.83$ & $21.37 \pm 0.97$ & $\bm{18.97 \pm 0.85}$ & $20.23 \pm 0.89$ & $20.37 \pm 0.95$ &  $20.08 \pm 0.91$ \\
\bottomrule \\
\end{tabular}
\caption{Noisy Imagenet Error Rates (VGG-19)}
\end{table}

\begin{table}[]
    \centering
\begin{tabular}{llll}
\toprule
          Model &              TS &             ETS &        imax sCW \\
\midrule
$1.60 \pm 0.10$ & $1.70 \pm 0.09$ & $1.75 \pm 0.08$ & $1.91 \pm 0.09$ \\
$0.98 \pm 0.09$ & $1.04 \pm 0.08$ & $1.07 \pm 0.08$ & $1.32 \pm 0.08$ \\
$1.09 \pm 0.10$ & $1.03 \pm 0.08$ & $1.05 \pm 0.07$ & $1.26 \pm 0.08$ \\
\midrule
$2.02 \pm 0.09$ & $2.11 \pm 0.08$ & $2.18 \pm 0.08$ & $2.32 \pm 0.07$ \\
$1.30 \pm 0.08$ & $1.37 \pm 0.08$ & $1.39 \pm 0.08$ & $1.64 \pm 0.07$ \\
$1.22 \pm 0.08$ & $1.17 \pm 0.07$ & $1.19 \pm 0.07$ & $1.42 \pm 0.08$ \\
\midrule
$2.72 \pm 0.11$ & $2.78 \pm 0.10$ & $2.90 \pm 0.10$ & $2.96 \pm 0.11$ \\
$1.93 \pm 0.10$ & $1.95 \pm 0.10$ & $2.01 \pm 0.10$ & $3.57 \pm 1.21$ \\
$1.47 \pm 0.08$ & $1.42 \pm 0.06$ & $1.44 \pm 0.06$ & $1.66 \pm 0.06$ \\
\midrule
$3.79 \pm 0.11$ & $3.78 \pm 0.08$ & $3.95 \pm 0.10$ & $3.70 \pm 0.23$ \\
$2.97 \pm 0.10$ & $2.93 \pm 0.09$ & $3.04 \pm 0.07$ & $3.00 \pm 0.08$ \\
$1.97 \pm 0.08$ & $1.91 \pm 0.07$ & $1.95 \pm 0.07$ & $2.18 \pm 0.09$ \\
\bottomrule
\end{tabular}
    \caption{Calibration error (model alone), VGG-19}
    \label{tab:my_label}
\end{table}

\begin{table}[!h]
    \centering
\begin{tabular}{lllll}
\toprule
       C-2xConf &         C-Nocal &            C-TS &           C-ETS &      C-imax sCW \\
\midrule
$0.75 \pm 0.05$ & $0.69 \pm 0.06$ & $0.66 \pm 0.06$ & $0.65 \pm 0.06$ & $0.67 \pm 0.06$ \\
$0.69 \pm 0.05$ & $0.54 \pm 0.05$ & $0.51 \pm 0.05$ & $0.52 \pm 0.05$ & $0.52 \pm 0.05$ \\
$0.66 \pm 0.06$ & $0.67 \pm 0.07$ & $0.50 \pm 0.05$ & $0.51 \pm 0.05$ & $0.88 \pm 0.06$ \\
$1.05 \pm 0.06$ & $1.01 \pm 0.08$ & $0.95 \pm 0.08$ & $0.94 \pm 0.08$ & $0.96 \pm 0.08$ \\
$1.01 \pm 0.05$ & $0.76 \pm 0.07$ & $0.73 \pm 0.07$ & $0.73 \pm 0.07$ & $0.73 \pm 0.07$ \\
$0.90 \pm 0.06$ & $0.85 \pm 0.06$ & $0.68 \pm 0.07$ & $0.68 \pm 0.07$ & $0.69 \pm 0.07$ \\
$1.59 \pm 0.10$ & $1.56 \pm 0.12$ & $1.41 \pm 0.11$ & $1.38 \pm 0.11$ & $1.41 \pm 0.11$ \\
$1.46 \pm 0.08$ & $1.24 \pm 0.09$ & $1.12 \pm 0.09$ & $1.10 \pm 0.10$ & $3.50 \pm 2.13$ \\
$1.27 \pm 0.08$ & $1.16 \pm 0.07$ & $0.93 \pm 0.07$ & $0.93 \pm 0.07$ & $0.94 \pm 0.08$ \\
$2.33 \pm 0.10$ & $2.78 \pm 0.12$ & $2.30 \pm 0.11$ & $2.18 \pm 0.11$ & $2.33 \pm 0.23$ \\
$2.16 \pm 0.09$ & $2.25 \pm 0.11$ & $1.89 \pm 0.09$ & $1.81 \pm 0.08$ & $1.89 \pm 0.10$ \\
$1.88 \pm 0.08$ & $1.72 \pm 0.09$ & $1.40 \pm 0.09$ & $1.39 \pm 0.08$ & $1.42 \pm 0.08$ \\
\bottomrule \\
\end{tabular}
    \caption{Calibration error ($10^{-2}$) of the combined predictions on Noisy ImageNet (VGG-19)}
\end{table}
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%% Maximum-Likelihood fit version of these tables
\section{Calibrate After Fitting Combination}
\subsection{CIFAR-10}
\begin{table}[!h]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{llccc|ccc}
        \toprule
        \multicolumn{2}{c}{} &
        \multicolumn{3}{c}{Uncalibrated Model} & 
        \multicolumn{3}{c}{Calibrated Model} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8}
         Metric & Model Name & Model & Comb. & Recal. Comb. & Model & Comb. & Recal. Comb. \\
        \midrule
        \multirow{4}{*}{ECE ($10^{-2}$)} 
        & ResNet-110 & $5.23 \pm 0.36$ &  $2.23 \pm 0.24$ &  $0.56 \pm 0.17$ &  $1.19 \pm 0.28$ &  $1.82 \pm 0.26$ &  $0.68 \pm 0.22$ \\
        & ResNet-164 &  $3.00 \pm 0.32$ &  $1.72 \pm 0.23$ &  $0.49 \pm 0.18$ &  $1.02 \pm 0.30$ &  $1.39 \pm 0.21$ &  $0.56 \pm 0.17$ \\
        & PreResNet-164 &  $3.03 \pm 0.29$ &  $1.95 \pm 0.19$ &  $0.52 \pm 0.16$ &  $0.70 \pm 0.20$ &  $1.22 \pm 0.23$ &  $0.47 \pm 0.15$ \\
        & DenseNet-BC &  $2.18 \pm 0.27$ &  $1.67 \pm 0.21$ &  $0.72 \pm 0.19$ &  $0.79 \pm 0.19$ &  $0.94 \pm 0.15$ &  $0.39 \pm 0.09$ \\
        \midrule
        \multirow{4}{*}{cwECE ($10^{-2}$)}
        & ResNet-110 &  $0.87 \pm 0.06$ &  $0.25 \pm 0.05$ &  $0.22 \pm 0.03$ &  $0.43 \pm 0.05$ &  $0.22 \pm 0.04$ &  $0.20 \pm 0.04$ \\
        & ResNet-164 &  $0.44 \pm 0.06$ &  $0.17 \pm 0.03$ &  $0.17 \pm 0.03$ &  $0.29 \pm 0.04$ &  $0.16 \pm 0.03$ &  $0.17 \pm 0.03$ \\
        & PreResNet-164 &  $0.44 \pm 0.04$ &  $0.15 \pm 0.03$ &  $0.16 \pm 0.02$ &  $0.27 \pm 0.03$ &  $0.16 \pm 0.03$ &  $0.17 \pm 0.03$ \\
        & DenseNet-BC &  $2.18 \pm 0.27$ &  $1.67 \pm 0.21$ &  $0.72 \pm 0.19$ &  $0.79 \pm 0.19$ &  $0.94 \pm 0.15$ &  $0.39 \pm 0.09$ \\
        \midrule
        \multirow{4}{*}{NLL}
        & ResNet-110 &  $0.40 \pm 0.02$ &  $0.41 \pm 0.08$ &  $0.27 \pm 0.05$ &  $0.34 \pm 0.01$ &  $0.40 \pm 0.10$ &  $0.32 \pm 0.07$ \\
        & ResNet-164 &  $0.24 \pm 0.02$ &  $0.32 \pm 0.09$ &  $0.20 \pm 0.05$ &  $0.19 \pm 0.01$ &  $0.36 \pm 0.10$ &  $0.27 \pm 0.07$ \\
        & PreResNet-164 &  $0.23 \pm 0.02$ &  $0.30 \pm 0.08$ &  $0.16 \pm 0.03$ &  $0.16 \pm 0.01$ &  $0.36 \pm 0.10$ &  $0.26 \pm 0.07$ \\
        & DenseNet-BC &  $0.17 \pm 0.01$ &  $0.37 \pm 0.10$ &  $0.19 \pm 0.05$ &  $0.12 \pm 0.01$ &  $0.35 \pm 0.10$ &  $0.25 \pm 0.07$ \\
        \bottomrule
    \end{tabular}
    } % end resize box
    \caption{ Calibration metrics comparing model alone, human-model combination, and recalibrated human-model combination. All calibration done via TS with ~5k labeled data points. The data used to recalibrate the combination is the same data used to fit the confusion matrix and model temperature.}
    \label{table:cifar_calibrate_after_combining}
\end{table}

\subsection{ImageNet}
\begin{table}[!h]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{llccc|ccc}
        \toprule
        \multicolumn{2}{c}{} &
        \multicolumn{3}{c}{Uncalibrated Model} & 
        \multicolumn{3}{c}{Calibrated Model} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8}
         Metric & Noise Level & Model & Comb. & Recal. Comb. & Model & Comb. & Recal. Comb. \\
        \midrule
        \multirow{4}{*}{ECE ($10^{-2}$)} 
        & 80 &   $8.57 \pm 0.55$ &   $5.39 \pm 0.49$ &  $1.32 \pm 0.31$ &  $2.27 \pm 0.47$ &  $3.50 \pm 0.42$ &  $1.51 \pm 0.37$ \\
        & 95 &   $8.96 \pm 0.48$ &   $6.13 \pm 0.40$ &  $1.55 \pm 0.28$ &  $1.86 \pm 0.57$ &  $4.71 \pm 0.42$ &  $1.80 \pm 0.47$ \\
        & 110 &   $9.76 \pm 0.53$ &   $8.09 \pm 0.52$ &  $1.58 \pm 0.33$ &  $2.59 \pm 0.43$ &  $5.34 \pm 0.50$ &  $2.00 \pm 0.47$ \\
        & 125 &  $11.81 \pm 0.64$ &  $10.92 \pm 0.55$ &  $2.23 \pm 0.50$ &  $2.63 \pm 0.61$ &  $5.95 \pm 0.61$ &  $2.10 \pm 0.60$ \\
        \midrule
        \multirow{4}{*}{cwECE ($10^{-2}$)}
        & 80 &  $0.96 \pm 0.06$ &  $0.66 \pm 0.06$ &  $0.71 \pm 0.04$ &  $1.03 \pm 0.05$ &  $0.52 \pm 0.05$ &  $0.51 \pm 0.04$ \\
        & 95 &  $1.10 \pm 0.05$ &  $0.82 \pm 0.05$ &  $0.82 \pm 0.04$ &  $1.15 \pm 0.05$ &  $0.67 \pm 0.04$ &  $0.63 \pm 0.05$ \\
        & 110 &  $1.37 \pm 0.06$ &  $1.19 \pm 0.06$ &  $1.08 \pm 0.05$ &  $1.39 \pm 0.05$ &  $0.92 \pm 0.06$ &  $0.89 \pm 0.06$ \\
        & 125 &  $1.97 \pm 0.06$ &  $1.74 \pm 0.07$ &  $1.58 \pm 0.05$ &  $1.91 \pm 0.06$ &  $1.42 \pm 0.07$ &  $1.37 \pm 0.05$ \\
        \midrule
        \multirow{4}{*}{NLL}
        & 80 &  $0.71 \pm 0.05$ &  $1.25 \pm 0.21$ &  $0.48 \pm 0.06$ &  $0.36 \pm 0.02$ &  $1.43 \pm 0.28$ &  $1.01 \pm 0.19$ \\
        & 95 &  $0.70 \pm 0.03$ &  $1.26 \pm 0.20$ &  $0.55 \pm 0.07$ &  $0.40 \pm 0.01$ &  $1.31 \pm 0.25$ &  $0.96 \pm 0.17$ \\
        & 110 &  $0.73 \pm 0.03$ &  $1.49 \pm 0.22$ &  $0.74 \pm 0.09$ &  $0.49 \pm 0.02$ &  $1.46 \pm 0.23$ &  $1.14 \pm 0.17$ \\
        & 125 &  $0.89 \pm 0.03$ &  $1.18 \pm 0.19$ &  $0.79 \pm 0.09$ &  $0.70 \pm 0.02$ &  $1.05 \pm 0.21$ &  $0.94 \pm 0.16$ \\
        \bottomrule
    \end{tabular}
    } % end resize box
    \caption{VGG-19 }
    \label{table:imagenet_vgg19_calibrate_after_combining}
\end{table}

\begin{table}[!h]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{llccc|ccc}
        \toprule
        \multicolumn{2}{c}{} &
        \multicolumn{3}{c}{Uncalibrated Model} & 
        \multicolumn{3}{c}{Calibrated Model} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8}
         Metric & Noise Level & Model & Comb. & Recal. Comb. & Model & Comb. & Recal. Comb. \\
        \midrule
        \multirow{4}{*}{ECE ($10^{-2}$)} 
        & 80 &   $7.40 \pm 0.58$ &   $4.53 \pm 0.48$ &  $1.35 \pm 0.30$ &  $1.63 \pm 0.29$ &  $3.95 \pm 0.36$ &  $1.65 \pm 0.38$ \\
        & 95 &   $9.23 \pm 0.58$ &   $6.03 \pm 0.47$ &  $1.76 \pm 0.46$ &  $2.40 \pm 0.44$ &  $4.58 \pm 0.41$ &  $1.63 \pm 0.39$ \\
        & 110 &   $9.26 \pm 0.66$ &   $7.85 \pm 0.50$ &  $1.49 \pm 0.34$ &  $2.58 \pm 0.46$ &  $5.41 \pm 0.40$ &  $1.88 \pm 0.50$ \\
        & 125 &  $11.98 \pm 0.40$ &  $11.03 \pm 0.61$ &  $2.38 \pm 0.65$ &  $3.13 \pm 0.41$ &  $6.97 \pm 0.46$ &  $2.89 \pm 0.38$ \\
        \midrule
        \multirow{4}{*}{cwECE ($10^{-2}$)}
        & 80 &  $1.33 \pm 0.07$ &  $0.72 \pm 0.05$ &  $0.74 \pm 0.04$ &  $1.36 \pm 0.06$ &  $0.60 \pm 0.04$ &  $0.59 \pm 0.03$ \\
        & 95 &  $1.48 \pm 0.07$ &  $0.91 \pm 0.06$ &  $0.91 \pm 0.06$ &  $1.49 \pm 0.06$ &  $0.76 \pm 0.05$ &  $0.75 \pm 0.06$ \\
        & 110 &  $1.69 \pm 0.08$ &  $1.27 \pm 0.06$ &  $1.18 \pm 0.06$ &  $1.68 \pm 0.07$ &  $1.06 \pm 0.06$ &  $1.02 \pm 0.06$ \\
        & 125 &  $2.31 \pm 0.06$ &  $1.93 \pm 0.06$ &  $1.74 \pm 0.07$ &  $2.27 \pm 0.05$ &  $1.59 \pm 0.06$ &  $1.53 \pm 0.06$ \\
        \midrule
        \multirow{4}{*}{NLL}
        & 80 &  $0.59 \pm 0.03$ &  $1.45 \pm 0.26$ &  $0.82 \pm 0.14$ &  $0.47 \pm 0.02$ &  $1.51 \pm 0.29$ &  $1.12 \pm 0.20$ \\
        & 95 &  $0.65 \pm 0.03$ &  $1.42 \pm 0.25$ &  $0.83 \pm 0.13$ &  $0.53 \pm 0.02$ &  $1.41 \pm 0.26$ &  $1.07 \pm 0.18$ \\
        & 110 &  $0.75 \pm 0.03$ &  $1.60 \pm 0.23$ &  $0.98 \pm 0.12$ &  $0.63 \pm 0.02$ &  $1.54 \pm 0.23$ &  $1.23 \pm 0.17$ \\
        & 125 &  $0.97 \pm 0.02$ &  $1.26 \pm 0.21$ &  $0.93 \pm 0.12$ &  $0.84 \pm 0.02$ &  $1.16 \pm 0.21$ &  $1.05 \pm 0.16$ \\
        \bottomrule
    \end{tabular}
    } % end resize box
    \caption{GoogLeNet}
    \label{table:imagenet_googlenet_calibrate_after_combining}
\end{table}


%%%%% Calibration metrics removed from Appendix C
\begin{table}[!h]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{llcccc}
        \toprule
        Metric & Model  &     Uncalibrated &               TS &              ETS &             IMax \\
        \midrule
        \multirow{4}{*}{ECE ($10^{-2}$)} 
        & ResNet-110    &  $5.23 \pm 0.36$ &  $\bm{1.19 \pm 0.28}$ &  $1.29 \pm 0.29$ &  $1.21 \pm 0.30$       \\
        & ResNet-164    &  $3.00 \pm 0.32$ &  $1.02 \pm 0.30$      &  $1.10 \pm 0.27$ &  $\bm{0.77 \pm 0.32}$  \\
        & PreResNet-164 &  $3.03 \pm 0.29$ &  $0.70 \pm 0.20$      &  $0.77 \pm 0.20$ &  $\bm{0.61 \pm 0.24}$  \\
        & DenseNet-BC   &  $2.18 \pm 0.27$ &  $0.79 \pm 0.19$      &  $1.04 \pm 0.23$ &  $\bm{0.50 \pm 0.22}$  \\
        \midrule
        \multirow{4}{*}{cwECE ($10^{-2}$)} 
        & ResNet-110 &  $0.87 \pm 0.06$ &  $0.43 \pm 0.05$ &  $0.46 \pm 0.05$ &  $\bm{0.40 \pm 0.05}$ \\
        & ResNet-164 &  $0.44 \pm 0.06$ &  $0.29 \pm 0.04$ &  $0.31 \pm 0.04$ &  $\bm{0.26 \pm 0.04}$ \\
        & PreResNet-164 &  $0.44 \pm 0.04$ &  $0.27 \pm 0.03$ &  $0.28 \pm 0.03$ &  $\bm{0.24 \pm 0.03}$ \\
        & DenseNet-BC &  $0.23 \pm 0.03$ &  $0.27 \pm 0.02$ &  $0.35 \pm 0.02$ &  $\bm{0.19 \pm 0.03}$ \\
        \midrule
        \multirow{4}{*}{NLL} 
        & ResNet-110 &  $0.40 \pm 0.02$ &  $\bm{0.34 \pm 0.01}$ &  $\bm{0.34 \pm 0.01}$ &  $0.35 \pm 0.01$ \\
        & ResNet-164 &  $0.24 \pm 0.02$ &  $\bm{0.19 \pm 0.01}$ &  $0.20 \pm 0.01$ &  $0.20 \pm 0.01$ \\
        & PreResNet-164 &  $0.23 \pm 0.02$ &  $\bm{0.16 \pm 0.01}$ &  $\bm{0.16 \pm 0.01}$ &  $0.17 \pm 0.01$ \\
        & DenseNet-BC &  $0.17 \pm 0.01$ &  $\bm{0.12 \pm 0.01}$ &  $0.13 \pm 0.01$ &  $0.13 \pm 0.01$ \\
        \bottomrule
    \end{tabular}
    } % end resize box
    \caption{Calibration metrics of the model alone (no combination), CIFAR-10 {\color{red} write caption}}
    \label{table:cifar10_calibration_model}
\end{table}

\begin{table}[!h]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{llccccc}
        \toprule
         Metric & Model & Confusion &    Uncalibrated &               TS &              ETS &             IMax \\
        \midrule
        \multirow{4}{*}{ECE ($10^{-2}$)} 
        & ResNet-110 &  $\bm{1.34 \pm 0.34}$ &  $2.23 \pm 0.24$ &  $1.82 \pm 0.26$ &  $1.74 \pm 0.25$ &  $1.89 \pm 0.25$ \\
        & ResNet-164 &  $\bm{1.23 \pm 0.32}$ &  $1.72 \pm 0.23$ &  $1.39 \pm 0.21$ &  $1.33 \pm 0.22$ &  $1.49 \pm 0.22$ \\
        & PreResNet-164 &  $1.20 \pm 0.31$ &  $1.95 \pm 0.19$ &  $1.22 \pm 0.23$ &  $\bm{1.19 \pm 0.24}$ &  $1.35 \pm 0.26$ \\
        & DenseNet-BC &  $0.93 \pm 0.29$ &  $1.67 \pm 0.21$ &  $0.94 \pm 0.15$ &  $\bm{0.92 \pm 0.15}$ &  $1.16 \pm 0.18$ \\
        \midrule
        \multirow{4}{*}{cwECE ($10^{-2}$)} 
        & ResNet-110 &  $0.31 \pm 0.05$ &  $0.25 \pm 0.05$ &  $\bm{0.22 \pm 0.04}$ &  $\bm{0.22 \pm 0.05}$ &  $\bm{0.22 \pm 0.05}$ \\
        & ResNet-164 &  $0.24 \pm 0.04$ &  $0.17 \pm 0.03$ &  $\bm{0.16 \pm 0.03}$ &  $0.17 \pm 0.03$ &  $0.17 \pm 0.03$ \\
        & PreResNet-164 &  $0.24 \pm 0.05$ &  $\bm{0.15 \pm 0.03}$ &  $0.16 \pm 0.03$ &  $0.16 \pm 0.03$ &  $\bm{0.15 \pm 0.02}$ \\
        & DenseNet-BC &  $0.20 \pm 0.03$ &  $0.14 \pm 0.02$ &  $\bm{0.13 \pm 0.02}$ &  $\bm{0.13 \pm 0.02}$ &  $\bm{0.13 \pm 0.02}$ \\
        \midrule
        \multirow{4}{*}{NLL}
        & ResNet-110 &  $0.66 \pm 0.14$ &  $0.41 \pm 0.08$ &  $\bm{0.40 \pm 0.10}$ &  $0.41 \pm 0.10$ &  $0.41 \pm 0.10$ \\
        & ResNet-164 &  $0.62 \pm 0.12$ &  $\bm{0.32 \pm 0.09}$ &  $0.36 \pm 0.10$ &  $0.37 \pm 0.10$ &  $0.37 \pm 0.10$ \\
        & PreResNet-164 &  $0.63 \pm 0.17$ &  $\bm{0.30 \pm 0.08}$ &  $0.36 \pm 0.10$ &  $0.36 \pm 0.10$ &  $0.37 \pm 0.10$ \\
        & DenseNet-BC &  $0.57 \pm 0.15$ &  $0.37 \pm 0.10$ &  $\bm{0.35 \pm 0.10}$ &  $\bm{0.35 \pm 0.10}$ &  $\bm{0.35 \pm 0.10}$ \\
        \bottomrule
    \end{tabular}
    } % end resize box
    \caption{Calibration metrics of the human-model combination, CIFAR-10, {\color{red} write caption} }
    \label{table:cifar10_calibration_comb}
\end{table}

\begin{table}[!h]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lccccc}
        \toprule
         Metric & Noise Level & Uncalibrated &               TS &              ETS &             IMax \\
        \midrule
        \multirow{4}{*}{ECE ($10^{-2}$)} 
        & 80 &   $8.57 \pm 0.55$ &  $2.27 \pm 0.47$ &  $2.26 \pm 0.43$ &  $\bm{1.06 \pm 0.38}$ \\
        & 95 &   $8.96 \pm 0.48$ &  $1.86 \pm 0.57$ &  $1.93 \pm 0.58$ &  $\bm{1.40 \pm 0.52}$ \\
        & 110 &   $9.76 \pm 0.53$ &  $2.59 \pm 0.43$ &  $2.69 \pm 0.45$ &  $\bm{1.52 \pm 0.42}$ \\
        & 125 &  $11.81 \pm 0.64$ &  $2.63 \pm 0.61$ &  $2.64 \pm 0.55$ &  $\bm{1.83 \pm 0.61}$ \\
        \midrule
        \multirow{4}{*}{cwECE ($10^{-2}$)} 
        & 80 &  $0.96 \pm 0.06$ &  $1.03 \pm 0.05$ &  $1.05 \pm 0.05$ &  $\bm{0.90 \pm 0.06}$ \\
        & 95 &  $1.10 \pm 0.05$ &  $1.15 \pm 0.05$ &  $1.17 \pm 0.05$ &  $\bm{1.06 \pm 0.06}$ \\
        & 110 &  $1.37 \pm 0.06$ &  $1.39 \pm 0.05$ &  $1.42 \pm 0.05$ &  $\bm{1.31 \pm 0.06}$ \\
        & 125 &  $1.97 \pm 0.06$ &  $1.91 \pm 0.06$ &  $1.95 \pm 0.05$ &  $\bm{1.85 \pm 0.06}$ \\
        \midrule
        \multirow{4}{*}{NLL}
        & 80 &  $0.71 \pm 0.05$ &  $\bm{0.36 \pm 0.02}$ &  $\bm{0.36 \pm 0.02}$ &  $0.40 \pm 0.02$ \\
        & 95 &  $0.70 \pm 0.03$ &  $\bm{0.40 \pm 0.01}$ &  $\bm{0.40 \pm 0.01}$ &  $0.44 \pm 0.02$ \\
        & 110 &  $0.73 \pm 0.03$ &  $\bm{0.49 \pm 0.02}$ &  $\bm{0.49 \pm 0.02}$ &  $0.52 \pm 0.02$ \\
        & 125 &  $0.89 \pm 0.03$ &  $\bm{0.70 \pm 0.02}$ &  $\bm{0.70 \pm 0.02}$ &  $0.74 \pm 0.02$ \\
        \bottomrule
    \end{tabular}
    } % end resize box
    \caption{Calibration metrics of the model alone, ImageNet VGG-19, {\color{red} write caption} }
    \label{table:imagenet_calibration_vgg19}
\end{table}

\begin{table}[!h]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lcccccc}
        \toprule
         Metric & Noise Level & Confusion & Uncalibrated &               TS &              ETS &             IMax \\
        \midrule
        \multirow{4}{*}{ECE ($10^{-2}$)} 
        & 80 &  $\bm{2.65 \pm 0.38}$ &   $5.39 \pm 0.49$ &  $3.50 \pm 0.42$ &  $3.70 \pm 0.41$ &  $3.50 \pm 0.44$ \\
        & 95 &  $\bm{3.24 \pm 0.50}$ &   $6.13 \pm 0.40$ &  $4.71 \pm 0.42$ &  $4.77 \pm 0.43$ &  $4.47 \pm 0.41$ \\
        & 110 &  $\bm{4.22 \pm 0.72}$ &   $8.09 \pm 0.52$ &  $5.34 \pm 0.50$ &  $5.27 \pm 0.51$ &  $5.19 \pm 0.50$ \\
        & 125 &  $\bm{4.99 \pm 0.67}$ &  $10.92 \pm 0.55$ &  $5.95 \pm 0.61$ &  $5.65 \pm 0.62$ &  $6.52 \pm 0.69$ \\
        \midrule
        \multirow{4}{*}{cwECE ($10^{-2}$)} 
        & 80 &  $\bm{0.34 \pm 0.05}$ &  $0.66 \pm 0.06$ &  $0.52 \pm 0.05$ &  $0.52 \pm 0.04$ &  $0.54 \pm 0.04$ \\
        & 95 &  $\bm{0.45 \pm 0.05}$ &  $0.82 \pm 0.05$ &  $0.67 \pm 0.04$ &  $0.68 \pm 0.04$ &  $0.68 \pm 0.04$ \\
        & 110 &  $\bm{0.59 \pm 0.07}$ &  $1.19 \pm 0.06$ &  $0.92 \pm 0.06$ &  $0.92 \pm 0.06$ &  $0.94 \pm 0.06$ \\
        & 125 &  $\bm{0.78 \pm 0.07}$ &  $1.74 \pm 0.07$ &  $1.42 \pm 0.07$ &  $1.41 \pm 0.06$ &  $1.43 \pm 0.07$ \\
        \midrule
        \multirow{4}{*}{NLL}
        & 80 &  $1.30 \pm 0.29$ &  $\bm{1.25 \pm 0.21}$ &  $1.43 \pm 0.28$ &  $1.47 \pm 0.28$ &  $1.50 \pm 0.29$ \\
        & 95 &  $\bm{1.22 \pm 0.24}$ &  $1.26 \pm 0.20$ &  $1.31 \pm 0.25$ &  $1.37 \pm 0.25$ &  $1.38 \pm 0.25$ \\
        & 110 &  $\bm{1.35 \pm 0.22}$ &  $1.49 \pm 0.22$ &  $1.46 \pm 0.23$ &  $1.47 \pm 0.23$ &  $1.48 \pm 0.23$ \\
        & 125 &  $1.12 \pm 0.24$ &  $1.18 \pm 0.19$ &  $\bm{1.05 \pm 0.21}$ &  $1.06 \pm 0.21$ &  $1.08 \pm 0.21$ \\
        \bottomrule
    \end{tabular}
    } % end resize box
    \caption{Calibration metrics of the combination, ImageNet VGG-19, {\color{red} write caption} }
    \label{table:imagenet_calibration_comb_vgg19}
\end{table}

\comment{ %%%%% Old version
\begin{table}[!h]
    \centering
    \begin{tabular}{lrrrrr}
    \toprule
    \multicolumn{2}{c}{Model Only} &
    \multicolumn{3}{c}{Combination} \\
    \cmidrule(lr){1-2}  \cmidrule(lr){3-5}
    Uncalibrated &  Calibrated & Confusion & Uncalibrated & Calibrated \\
    \midrule 
    $1.09 \pm 0.10$ & $1.03 \pm 0.08$ & $0.66 \pm 0.06$ & $0.67 \pm 0.07$ & $\bm{0.50 \pm 0.05}$ \\
    $1.22 \pm 0.08$ & $1.17 \pm 0.07$ & $0.90 \pm 0.06$ & $0.85 \pm 0.06$ & $\bm{0.68 \pm 0.07}$ \\
    $1.47 \pm 0.08$ & $1.42 \pm 0.06$ & $1.27 \pm 0.08$ & $1.16 \pm 0.07$ & $\bm{0.93 \pm 0.07}$ \\
    $1.97 \pm 0.08$ & $1.91 \pm 0.07$ & $1.88 \pm 0.08$ & $1.72 \pm 0.09$ & $\bm{1.40 \pm 0.09}$ \\
    \bottomrule \\
    \end{tabular}
    \caption{Calibration error ($10^{-2}$) for combination and various baseline models on Noisy ImageNet. The calibration method used was temperature scaling. {\color{red} update this using different calibration metric}}
    \label{table:imagenet_ce}
\end{table}
}


\comment{ %%%%%% Old version of VGG-19 error rates
\begin{table}[!h]
    \centering
    \begin{tabular}{lcrrrr}
    \toprule
    \multicolumn{2}{c}{} &
    \multicolumn{5}{c}{Combination} \\
    \cmidrule(lr){2-7}
    Human & Model & Confusion & Uncalibrated & TS &  ETS & IMax \\
    \midrule 
    9.85  & $11.03 \pm 0.89$ &  $6.49  \pm 0.56$ &  $7.34 \pm 0.58$ &  $\bm{6.38 \pm 0.60}$ \\
    14.07 & $12.82 \pm 0.92$ &  $9.15  \pm 0.62$ &  $9.08 \pm 0.55$ &  $\bm{9.07 \pm 0.59}$ \\
    23.34 & $15.85 \pm 0.73$ &  $14.23 \pm 0.83$ & $\bm{12.64 \pm 0.76}$ & $13.10 \pm 0.85$ \\
    39.77 & $21.68 \pm 0.83$ &  $21.37 \pm 0.97$ & $\bm{18.97 \pm 0.85}$ & $20.23 \pm 0.89$ \\
    \bottomrule \\
    \end{tabular}
    \caption{Error rates (\%, $\pm$ one standard deviation) for VGG-19 on Noisy ImageNet.}
    \label{table:imagenet_error_rates}
\end{table}
}

\begin{table}[!h]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lccccc}
        \toprule
         Metric & Noise Level & Uncalibrated &               TS &              ETS &             IMax \\
        \midrule
        \multirow{4}{*}{ECE ($10^{-2}$)} 
        & 80 &   $7.40 \pm 0.58$ &  $1.63 \pm 0.29$ &  $1.74 \pm 0.41$ &  $\bm{1.58 \pm 0.45}$ \\
        & 95 &   $9.23 \pm 0.58$ &  $2.40 \pm 0.44$ &  $2.32 \pm 0.41$ &  $\bm{1.53 \pm 0.49}$ \\
        & 110 &   $9.26 \pm 0.66$ &  $2.58 \pm 0.46$ &  $2.66 \pm 0.50$ &  $\bm{1.59 \pm 0.51}$ \\
        & 125 &  $11.98 \pm 0.40$ &  $3.13 \pm 0.41$ &  $3.13 \pm 0.53$ &  $\bm{1.88 \pm 0.49}$ \\
        \midrule
        \multirow{4}{*}{cwECE ($10^{-2}$)} 
        & 80 &  $1.33 \pm 0.07$ &  $1.36 \pm 0.06$ &  $1.39 \pm 0.06$ &  $\bm{1.29 \pm 0.07}$ \\
        & 95 &  $1.48 \pm 0.07$ &  $1.49 \pm 0.06$ &  $1.52 \pm 0.07$ &  $\bm{1.41 \pm 0.07}$ \\
        & 110 &  $1.69 \pm 0.08$ &  $1.68 \pm 0.07$ &  $1.70 \pm 0.07$ &  $\bm{1.59 \pm 0.08}$ \\
        & 125 &  $2.31 \pm 0.06$ &  $2.27 \pm 0.05$ &  $2.31 \pm 0.05$ &  $\bm{2.10 \pm 0.06}$ \\
        \midrule
        \multirow{4}{*}{NLL}
        & 80 &  $0.59 \pm 0.03$ &  $\bm{0.47 \pm 0.02}$ &  $\bm{0.47 \pm 0.02}$ &  $0.48 \pm 0.02$ \\
        & 95 &  $0.65 \pm 0.03$ &  $\bm{0.53 \pm 0.02}$ &  $\bm{0.53 \pm 0.02}$ &  $0.54 \pm 0.02$ \\
        & 110 &  $0.75 \pm 0.03$ &  $\bm{0.63 \pm 0.02}$ &  $\bm{0.63 \pm 0.02}$ &  $0.64 \pm 0.02$ \\
        & 125 &  $0.97 \pm 0.02$ &  $\bm{0.84 \pm 0.02}$ &  $\bm{0.84 \pm 0.02}$ &  $0.85 \pm 0.02$ \\
        \bottomrule
    \end{tabular}
    } % end resize box
    \caption{Calibration metrics of the model alone, ImageNet GoogLeNet, {\color{red} write caption} }
    \label{table:imagenet_calibration_googlenet}
\end{table}

\begin{table}[!h]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lcccccc}
        \toprule
         Metric & Noise Level & Confusion & Uncalibrated &               TS &              ETS &             IMax \\
        \midrule
        \multirow{4}{*}{ECE ($10^{-2}$)} 
        & 80 &  $\bm{2.66 \pm 0.41}$ &   $4.53 \pm 0.48$ &  $3.95 \pm 0.36$ &  $3.99 \pm 0.36$ &  $4.20 \pm 0.38$ \\
        & 95 &  $\bm{3.27 \pm 0.61}$ &   $6.03 \pm 0.47$ &  $4.58 \pm 0.41$ &  $4.59 \pm 0.46$ &  $4.86 \pm 0.44$ \\
        & 110 &  $\bm{4.40 \pm 0.70}$ &   $7.85 \pm 0.50$ &  $5.41 \pm 0.40$ &  $5.44 \pm 0.39$ &  $5.86 \pm 0.43$ \\
        & 125 &  $\bm{5.94 \pm 0.60}$ &  $11.03 \pm 0.61$ &  $6.97 \pm 0.46$ &  $6.84 \pm 0.47$ &  $7.53 \pm 0.56$ \\
        \midrule
        \multirow{4}{*}{cwECE ($10^{-2}$)} 
        & 80 &  $\bm{0.37 \pm 0.04}$ &  $0.72 \pm 0.05$ &  $0.60 \pm 0.04$ &  $0.59 \pm 0.04$ &  $0.60 \pm 0.04$ \\
        & 95 &  $\bm{0.49 \pm 0.07}$ &  $0.91 \pm 0.06$ &  $0.76 \pm 0.05$ &  $0.75 \pm 0.05$ &  $0.76 \pm 0.05$ \\
        & 110 &  $\bm{0.66 \pm 0.08}$ &  $1.27 \pm 0.06$ &  $1.06 \pm 0.06$ &  $1.05 \pm 0.07$ &  $1.07 \pm 0.06$ \\
        & 125 &  $\bm{0.96 \pm 0.08}$ &  $1.93 \pm 0.06$ &  $1.59 \pm 0.06$ &  $1.56 \pm 0.07$ &  $1.61 \pm 0.07$ \\
        \midrule
        \multirow{4}{*}{NLL}
        & 80 &  $\bm{1.33 \pm 0.24}$ &  $1.45 \pm 0.26$ &  $1.51 \pm 0.29$ &  $1.52 \pm 0.29$ &  $1.52 \pm 0.29$ \\
        & 95 &  $\bm{1.41 \pm 0.28}$ &  $1.42 \pm 0.25$ &  $\bm{1.41 \pm 0.26}$ &  $\bm{1.41 \pm 0.26}$ &  $\bm{1.41 \pm 0.26}$ \\
        & 110 &  $1.56 \pm 0.25$ &  $1.60 \pm 0.23$ &  $\bm{1.54 \pm 0.23}$ &  $\bm{1.54 \pm 0.23}$ &  $1.55 \pm 0.23$ \\
        & 125 &  $1.25 \pm 0.22$ &  $1.26 \pm 0.21$ &  $\bm{1.16 \pm 0.21}$ &  $\bm{1.16 \pm 0.21}$ &  $1.17 \pm 0.21$ \\
        \bottomrule
    \end{tabular}
    } % end resize box
    \caption{Calibration metrics of the combination, ImageNet GoogLeNet, {\color{red} write caption} }
    \label{table:imagenet_calibration_comb_googlenet}
\end{table}


%%%%%%%%%%%%%% Old version of calibrate after combining tables

\begin{table}[!h]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{llccc|ccc}
        \toprule
        \multicolumn{2}{c}{} &
        \multicolumn{3}{c}{Uncalibrated Model} & 
        \multicolumn{3}{c}{Calibrated Model} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8}
         Metric & Model Name & Model & Comb. & Recal. Comb. & Model & Comb. & Recal. Comb. \\
        \midrule
        \multirow{4}{*}{ECE ($10^{-2}$)} 
        & ResNet-110 &  $5.23 \pm 0.35$ &  $2.08 \pm 0.25$ &  $1.30 \pm 0.22$ &  $3.04 \pm 0.37$ &  $1.68 \pm 0.23$ &  $0.84 \pm 0.18$ \\
        & ResNet-164 &  $2.98 \pm 0.34$ &  $1.63 \pm 0.23$ &  $1.17 \pm 0.24$ &  $1.92 \pm 0.28$ &  $1.36 \pm 0.20$ &  $0.84 \pm 0.20$ \\
        & PreResNet-164 &  $3.03 \pm 0.29$ &  $1.87 \pm 0.22$ &  $1.55 \pm 0.21$ &  $2.26 \pm 0.27$ &  $1.41 \pm 0.20$ &  $1.05 \pm 0.21$ \\
        & DenseNet-BC &  $2.18 \pm 0.27$ &  $1.53 \pm 0.20$ &  $1.32 \pm 0.19$ &  $1.69 \pm 0.27$ &  $1.24 \pm 0.17$ &  $0.94 \pm 0.17$ \\
        \midrule
        \multirow{4}{*}{cwECE ($10^{-2}$)}
        & ResNet-110 &  $0.81 \pm 0.07$ &  $0.23 \pm 0.05$ &  $0.21 \pm 0.05$ &  $0.60 \pm 0.06$ &  $0.20 \pm 0.05$ &  $0.18 \pm 0.04$ \\
        & ResNet-164 &  $0.39 \pm 0.06$ &  $0.15 \pm 0.03$ &  $0.15 \pm 0.03$ &  $0.34 \pm 0.05$ &  $0.14 \pm 0.03$ &  $0.14 \pm 0.03$ \\
        & PreResNet-164 &  $0.29 \pm 0.04$ &  $0.13 \pm 0.03$ &  $0.13 \pm 0.03$ &  $0.28 \pm 0.03$ &  $0.13 \pm 0.03$ &  $0.13 \pm 0.03$ \\
        & DenseNet-BC &  $0.23 \pm 0.03$ &  $0.11 \pm 0.02$ &  $0.11 \pm 0.02$ &  $0.23 \pm 0.03$ &  $0.10 \pm 0.02$ &  $0.10 \pm 0.02$ \\
        \midrule
        \multirow{4}{*}{NLL}
        &  ResNet-110 &  $0.40 \pm 0.02$ &  $0.16 \pm 0.01$ &  $0.14 \pm 0.01$ &  $0.35 \pm 0.02$ &  $0.14 \pm 0.01$ &  $0.12 \pm 0.01$ \\
        & ResNet-164 &  $0.24 \pm 0.02$ &  $0.11 \pm 0.01$ &  $0.10 \pm 0.01$ &  $0.21 \pm 0.01$ &  $0.10 \pm 0.01$ &  $0.09 \pm 0.01$ \\
        &  PreResNet-164 &  $0.23 \pm 0.02$ &  $0.13 \pm 0.02$ &  $0.10 \pm 0.01$ &  $0.19 \pm 0.01$ &  $0.10 \pm 0.01$ &  $0.08 \pm 0.01$ \\
        & DenseNet-BC &  $0.17 \pm 0.01$ &  $0.10 \pm 0.01$ &  $0.08 \pm 0.01$ &  $0.14 \pm 0.01$ &  $0.08 \pm 0.01$ &  $0.07 \pm 0.01$ \\
        \bottomrule
    \end{tabular}
    } % end resize box
    \caption{ Calibration metrics comparing model alone, human-model combination, and recalibrated human-model combination. All calibration done via TS with ~5k labeled data points. The data used to recalibrate the combination is the same data used to fit the confusion matrix and model temperature. All fits are MAP.}
    \label{table:cifar_calibrate_after_combining}
\end{table}

\begin{table}[!h]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{llccc|ccc}
        \toprule
        \multicolumn{2}{c}{} &
        \multicolumn{3}{c}{Uncalibrated Model} & 
        \multicolumn{3}{c}{Calibrated Model} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8}
         Metric & Noise Level & Model & Comb. & Recal. Comb. & Model & Comb. & Recal. Comb. \\
        \midrule
        \multirow{4}{*}{ECE ($10^{-2}$)} 
        & 80 &   $8.54 \pm 0.54$ &   $5.17 \pm 0.49$ &  $4.43 \pm 0.47$ &  $7.29 \pm 0.52$ &  $4.06 \pm 0.42$ &  $3.16 \pm 0.42$ \\
        & 95 &   $8.96 \pm 0.48$ &   $5.74 \pm 0.38$ &  $4.65 \pm 0.38$ &  $7.29 \pm 0.46$ &  $4.52 \pm 0.39$ &  $3.24 \pm 0.37$ \\
        & 110 &   $9.76 \pm 0.53$ &   $7.83 \pm 0.48$ &  $6.09 \pm 0.49$ &  $7.27 \pm 0.52$ &  $6.05 \pm 0.46$ &  $3.91 \pm 0.49$ \\
        & 125 &  $11.81 \pm 0.64$ &  $10.86 \pm 0.56$ &  $7.32 \pm 0.61$ &  $7.52 \pm 0.66$ &  $8.49 \pm 0.61$ &  $4.49 \pm 0.61$ \\
        \midrule
        \multirow{4}{*}{cwECE ($10^{-2}$)}
        & 80 &  $1.10 \pm 0.07$ &  $0.68 \pm 0.05$ &  $0.66 \pm 0.05$ &  $1.05 \pm 0.06$ &  $0.58 \pm 0.05$ &  $0.56 \pm 0.04$ \\
        & 95 &  $1.18 \pm 0.06$ &  $0.82 \pm 0.05$ &  $0.79 \pm 0.05$ &  $1.13 \pm 0.05$ &  $0.72 \pm 0.05$ &  $0.69 \pm 0.04$ \\
        & 110 &  $1.44 \pm 0.06$ &  $1.14 \pm 0.06$ &  $1.08 \pm 0.05$ &  $1.36 \pm 0.06$ &  $1.02 \pm 0.06$ &  $0.96 \pm 0.05$ \\
        & 125 &  $1.98 \pm 0.06$ &  $1.73 \pm 0.07$ &  $1.60 \pm 0.07$ &  $1.88 \pm 0.06$ &  $1.54 \pm 0.07$ &  $1.45 \pm 0.06$ \\
        \midrule
        \multirow{4}{*}{NLL}
        &  80 &  $0.71 \pm 0.05$ &  $0.49 \pm 0.04$ &  $0.37 \pm 0.03$ &  $0.52 \pm 0.03$ &  $0.34 \pm 0.03$ &  $0.27 \pm 0.02$ \\
        & 95 &  $0.70 \pm 0.03$ &  $0.52 \pm 0.03$ &  $0.40 \pm 0.02$ &  $0.53 \pm 0.03$ &  $0.39 \pm 0.02$ &  $0.32 \pm 0.02$ \\
        & 110 &  $0.73 \pm 0.03$ &  $0.61 \pm 0.04$ &  $0.48 \pm 0.03$ &  $0.58 \pm 0.02$ &  $0.49 \pm 0.03$ &  $0.41 \pm 0.02$ \\
        & 1125 &  $0.89 \pm 0.03$ &  $0.83 \pm 0.04$ &  $0.69 \pm 0.03$ &  $0.75 \pm 0.03$ &  $0.71 \pm 0.03$ &  $0.64 \pm 0.02$ \\
        \bottomrule
    \end{tabular}
    } % end resize box
    \caption{VGG-19 }
    \label{table:imagenet_vgg19_calibrate_after_combining}
\end{table}

\begin{table}[!h]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{llccc|ccc}
        \toprule
        \multicolumn{2}{c}{} &
        \multicolumn{3}{c}{Uncalibrated Model} & 
        \multicolumn{3}{c}{Calibrated Model} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8}
         Metric & Noise Level & Model & Comb. & Recal. Comb. & Model & Comb. & Recal. Comb. \\
        \midrule
        \multirow{4}{*}{ECE ($10^{-2}$)} 
        & 80 &   $7.39 \pm 0.58$ &   $4.10 \pm 0.46$ &  $2.86 \pm 0.42$ &  $4.54 \pm 0.58$ &  $3.27 \pm 0.47$ &  $1.96 \pm 0.39$ \\
        & 95 &   $9.23 \pm 0.58$ &   $5.68 \pm 0.42$ &  $3.89 \pm 0.45$ &  $5.86 \pm 0.59$ &  $4.48 \pm 0.42$ &  $2.53 \pm 0.41$ \\
        & 110 &   $9.04 \pm 0.68$ &   $7.58 \pm 0.46$ &  $5.00 \pm 0.45$ &  $5.15 \pm 0.61$ &  $5.88 \pm 0.44$ &  $2.98 \pm 0.43$ \\
        & 125 &  $11.98 \pm 0.40$ &  $10.97 \pm 0.60$ &  $6.49 \pm 0.59$ &  $6.59 \pm 0.38$ &  $8.00 \pm 0.53$ &  $3.37 \pm 0.41$ \\
        \midrule
        \multirow{4}{*}{cwECE ($10^{-2}$)}
        & 80 &  $1.33 \pm 0.07$ &  $0.67 \pm 0.04$ &  $0.66 \pm 0.04$ &  $1.30 \pm 0.06$ &  $0.58 \pm 0.03$ &  $0.57 \pm 0.03$ \\
        & 95 &  $1.47 \pm 0.08$ &  $0.87 \pm 0.06$ &  $0.83 \pm 0.05$ &  $1.44 \pm 0.07$ &  $0.76 \pm 0.04$ &  $0.74 \pm 0.05$ \\
        & 110 &  $1.70 \pm 0.08$ &  $1.23 \pm 0.06$ &  $1.15 \pm 0.06$ &  $1.63 \pm 0.07$ &  $1.11 \pm 0.06$ &  $1.03 \pm 0.06$ \\
        & 125 &  $2.31 \pm 0.06$ &  $1.92 \pm 0.06$ &  $1.75 \pm 0.06$ &  $2.21 \pm 0.06$ &  $1.72 \pm 0.06$ &  $1.59 \pm 0.06$ \\
        \midrule
        \multirow{4}{*}{NLL}
        & 80 &  $0.59 \pm 0.03$ &  $0.34 \pm 0.02$ &  $0.28 \pm 0.02$ &  $0.50 \pm 0.02$ &  $0.29 \pm 0.02$ &  $0.25 \pm 0.02$ \\
        & 95 &  $0.65 \pm 0.03$ &  $0.43 \pm 0.03$ &  $0.36 \pm 0.02$ &  $0.56 \pm 0.02$ &  $0.37 \pm 0.02$ &  $0.33 \pm 0.02$ \\
        & 110 &  $0.75 \pm 0.03$ &  $0.60 \pm 0.03$ &  $0.50 \pm 0.02$ &  $0.65 \pm 0.02$ &  $0.53 \pm 0.03$ &  $0.47 \pm 0.02$ \\
        & 125 &  $0.97 \pm 0.02$ &  $0.88 \pm 0.03$ &  $0.76 \pm 0.02$ &  $0.86 \pm 0.02$ &  $0.80 \pm 0.03$ &  $0.74 \pm 0.02$ \\
        \bottomrule
    \end{tabular}
    } % end resize box
    \caption{GoogLeNet}
    \label{table:imagenet_googlenet_calibrate_after_combining}
\end{table}

